Unpacking Human Teachers' Intentions For Natural Interactive Task Learning

Interactive Task Learning (ITL) is an emerging research agenda that studies the design of complex intelligent robots that can acquire new knowledge through natural human teacher-robot learner interactions. ITL methods are particularly useful for designing intelligent robots whose behavior can be adapted by humans collaborating with them. Various research communities are contributing methods for ITL and a large subset of this research is \emph{robot-centered} with a focus on developing algorithms that can learn online, quickly. This paper studies the ITL problem from a \emph{human-centered} perspective to provide guidance for robot design so that human teachers can naturally teach ITL robots. In this paper, we present 1) a qualitative bidirectional analysis of an interactive teaching study (N=10) through which we characterize various aspects of actions intended and executed by human teachers when teaching a robot; 2) an in-depth discussion of the teaching approach employed by two participants to understand the need for personal adaptation to individual teaching styles; and 3) requirements for ITL robot design based on our analyses and informed by a computational theory of collaborative interactions, SharedPlans.

==> 03_preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}
%/\begin{figure*}
%/\begin{subfigure}{.48\textwidth}
 % \centering
%  \includegraphics[width=.8\linewidth]{images/aileen/teach-box-new.png}  
%  \caption{A robot is shown a \emph{red box}.}
%  \label{fig:sub-first}
%\end{subfigure}
%\begin{subfigure}{.48\textwidth}
%  \centering
%  % include second image
%  \includegraphics[width=.8\linewidth]{images/aileen/teach-right-of-new.png}  
%  \caption{ A robot is shown that a red box is to the \emph{right of} a red cone.}
%  \label{fig:sub-second}
%\end{subfigure}

%\begin{subfigure}{.33\textwidth}
% \centering
%  % include third image
%   \includegraphics[width=.8\linewidth]{images/aileen/teach-move-1-new.png}  
%  \caption{Initial state: A blue cylinder is to the right of a red box.}
%  \label{fig:sub-third}
%\end{subfigure}
%\begin{subfigure}{.33\textwidth}
%  \centering
%  % include fourth image
%  \includegraphics[width=.8\linewidth]{images/aileen/teach-move-2-new.png}  
%  \caption{The instructor guides the robot to move the red box.}
%  \label{fig:sub-fourth}
%\end{subfigure}
%\begin{subfigure}{.33\textwidth}
%  \centering
%  % include fourth image
%  \includegraphics[width=.8\linewidth]{images/aileen/teach-move-3-new.png}  
%  \caption{Goal state: The red box is to the right of the blue cylinder.}
%  \label{fig:sub-fifth}
%\end{subfigure}
%\caption{After learning concepts such as `red', `box', and `right of' through configurations such as Figure \ref{fig:sub-first} and \ref{fig:sub-second}, the instructor demonstrates a move action as presented in Figure \ref{fig:sub-third}, \ref{fig:sub-fourth}, and \ref{fig:sub-fifth} so that \textsc{Aileen} can learn the \emph{move} action.}
%\label{fig:aileen-examples}
%\end{figure*}

Our research studies and develops interaction mechanisms for ITL robots that are designed using the cognitive systems paradigm. Cognitive systems are a class of AI systems that implement a variety of intelligent algorithms (such as search and planning, task-oriented dialog, goal-oriented reasoning, computer vision, multi-modal language processing etc.) in a single integrated system. In contrast to machine learning systems based on the deep neural network paradigm (that learn in batch mode during training), ITL robots have demonstrated end-to-end, online, task learning from small number of examples. \textsc{Aileen} \cite{mohan2020characterizing} is an ITL robot that has been built using the Soar cognitive architecture  \cite{laird2012soar} which has been augmented with deep learning architectures for low-level vision as well as models of analogical processing for high-level concept acquisition and generalization. It can learn novel concepts belonging to different parts of the domain ontology including visual concepts such as colors (\emph{red}) and shapes (\emph{box}); spatial concepts such as configurations (\emph{blue cylinder is to the right of the red box}); and action concepts (\emph{move the red box to the right of the blue cylinder}). Our work shows that these concepts not only are useful in scene understanding, they also support task planning and execution. While \textsc{Aileen} and other ITL agents have been shown have complex behavior, the research has taken a \emph{robot-learner}-centered view focusing on computational methods that enable interactive learning. This paper takes a different but aligned direction - we adopt a \emph{human-teacher}-centered view and study the nature of human teaching with a goal of designing robust interaction models that can learn from the wide range of information available in human teaching. 

%\textsc{Rosie} - an ITL system built in the Soar cognitive architecture \cite{laird2012soar} - can learn over $60$ games and puzzles \cite{kirk2016learning} and several mobile delivery and navigation tasks \cite{mininger2016interactively} through a combination of situated natural language commands and demonstrations. 

%\subsection{AILEEN}
%\textsc{Aileen} learns new domain \textbf{concepts} (shown in Figure \ref{fig:aileen-examples}) through situated interactions with a teacher. It can learn novel visual concepts such as colors (\emph{red}) and shapes (\emph{box}); spatial concepts such as configurations (\emph{blue cylinder is to the right of the red box}); and action concepts (\emph{move the red box to the right of the blue cylinder}). Visual and spatial concepts support scene understanding in \textsc{Aileen} via reasoning and inference mechanisms implemented over primitive visual and spatial classification. For example, if \textsc{Aileen} knows that a specific visual classification \texttt{CVc24} is correlated with the color \emph{red}, it can infer the color whenever it perceives a segmented object with this classification symbol. Spatial and action concepts support task execution through hierarchical, goal-oriented action-selection implemented over primitive control policies. For example, if \textsc{Aileen} knows that \emph{right-of} implies that \emph{red box} is to the east of and disconnected with \emph{blue cylinder}, it can plan a sequence of primitive \texttt{pick-up} and \texttt{place} control policies to achieve this goal.  

%Learning occurs through a sequence of \textbf{lessons} comprising conjoint stimuli of a situation and a linguistic utterance. The teacher generates static scenes by setting up objects to demonstrate visual and spatial concepts. Figures \ref{fig:sub-first} and \ref{fig:sub-second} show the scenes generated by the teacher in the Webots \textcolor{blue}{robot simulator} environment to teach \textsc{Aileen} how to interpret \emph{red box} and \emph{right of} respectively. A sequence of scenes that show temporal changes in the configuration of objects is used to demonstrate an action. For example, Figures \ref{fig:sub-third}, \ref{fig:sub-fourth}, and \ref{fig:sub-fifth} show an action trace for the verb \emph{move}.  \textsc{Aileen} thus jointly learns concept representations and the language to describe them. \textsc{Aileen} employs analogical reasoning and generalization to learn concepts and prior work has demonstrated that learned concept definitions enable language understanding as well as task execution \cite{mohan2020characterizing}. 

%\textsc{Aileen} learns from a sequence of lessons - a \textbf{curriculum} - that a teacher constructs to incrementally introduce various concepts relevant to the domain, and extracts generalizable knowledge from its experience. While \textsc{Aileen} has demonstrated flexible grounded concept learning, previous research has been \emph{robot-centered}, largely focusing on designing general methods to learn concepts incrementally. The exchange of information tends to be uni-directional, with the teacher structuring \textsc{Aileen}'s learning experiences. 


\subsection{SharedPlans}
\label{sec:sharedplans}
Past work in designing ITL robots such as \textsc{Aileen} has been forced to limit robot interactions, often requiring them to be scripted and restricted to a human teacher presenting examples, answering questions, or responding to requests by the robot. Based on everyday experience, it is clear that a good teacher adjusts teaching to a particular student's background and progress. To learn from the full range of information and structure in human teaching, it is desirable that a robot can engage in complex and flexible tutorial dialog. We view ITL as a process of teacher-student collaboration in which a human teacher and a student robot comprise a team and each works together to help the student learn a particular body of material. Problems or obstacles to this learning vary from student to student. Hence, they cannot be predicted and must be dynamically overcome during teaching. For these reasons, we explore a task-oriented, plan-based model of dialog processing \cite{grosz1986attention} which views dialog as emerging from collaboration. This paper explores how a particularly well-developed theory of collaboration called SharedPlans \cite{grosz-kraus, lochbaum-1998-collaborative, hunsberger, ortiz-dial, ortiz-dis} can be used to build robots that can flexibly collaborate with a teacher during ITL. %Previous research \cite{rich1998collagen, rickel2001building, Mohan2012} has shown that SharedPlans provides useful guidance for designing interaction models for agents with complex reasoning and behavior and consequently, is a useful paradigm to explore for ITL robots. 

SharedPlans posits that exchanges between participants are intentional and reflect the evolution of their mental states during collaboration. Each participant has a repertoire of \textbf{communicative actions} that they can choose from to make progress towards their joint, collaborative goals. Consider an ITL scenario in which a human teacher and \textsc{Aileen} have a collaborative goal for \textsc{Aileen} to learn how to \emph{build a wall} (Figure \ref{fig:study-env}) in its environment. Both participants - the teacher and the learner robot - will apply a series of communicative actions in service of this goal. Communicative actions vary and are selected in accordance with a participant's \textbf{intentions}. They include linguistic utterances accompanied with gestures. For instance, the teacher may intend \textsc{Aileen} to develop a shared belief that a particular object is of type \emph{box} and applies the communicative action of pointing to an object and saying \emph{this is a box}. Communicative actions also include actual physical actions in the environment. For example, upon being asked by the teacher, \textsc{Aileen} can adopt an intention to move an object and place it on a desired location on the table. 

Framing ITL exchanges as SharedPlans constructs, a \emph{lesson} can be considered as a sequence of communicative acts undertaken by the participants to achieve a collaborative goal of learning a relevant visual, spatial, or action \emph{concept} correctly. A \emph{curriculum}, then, is a sequence of lessons to achieve the overall collaborative goal of \textsc{Aileen} learning how to build a wall. The rest of the paper explores which intentions, communicative actions, and goals are useful to represent in an ITL agent such as \textsc{Aileen} (Sections \ref{sec:method} and \ref{sec:task-analysis}) and analyzes how SharedPlans can be used for managing ITL interactions (Section \ref{sec:discourse-analysis}) and learning from a variety of curricula that different people may employ.  

%In fact, historically, much of the early research in dialogue sprung from applications such as master-apprentice dialogues.  In those cases the master's role was to help the apprentice solve a particular task, such as the repairing of some piece of equipment.  In our setting, the role of the teacher is more persistent and the teaching is more structured, not focusing on one-off instances, but rather broad improvements by a student on some subject matter.
%These two characteristics, the inherent improvisational nature of the teacher-student interaction combined with the persistent role that a teacher plays, distinguish what we call {\it collaborative learning} from either collaborative dialogue or collaborative planning.
%Modeling such interactions as a collaboration follows work in plan-based dialogue management \cite{grosz1986attention, grosz-psych}.

%A collaboration involves the joint execution of some task; in our case, the task can involve learning the steps in some process, such as building a wall, or the teacher-induced task reflecting the sequencing of steps in a lesson, such as the presentation of material, evaluating progress and expanding of a student's knowledge.  SharedPlans places an emphasis on the ways in which the evolution of the mental states of the participants reflects the stages of a collaboration.  For example, if the goal of a lesson is for a student to learn how to make a wall, then the participants will, just as in a dialogue, share beliefs that will enable a plan to achieve that goal. The teacher will try to learn the student's beliefs or understanding of concepts in a lesson so that it can tailor the lesson for the student and the student will try to learn the information or beliefs communicated by the teacher about the domain during the lesson.  In the case of collaborative learning, if the student feels that the teacher is not addressing a problem then it is up to the student to speak up; similarly, if the teacher believes that the student is not progressing as planned it is up to the teacher to modify the lesson accordingly. In each case, a participant is helping by removing an obstacle to the successful execution of the goal and also adopting a {\it commitment} to do so over the course of the interaction.  Such commitments are called {\it intentions} \cite{brachman}. In a dialogue, such intentions are meant to be recognized by the other participant\footnote{In passing, it is mentioned in \cite{grosz-sidner} that in a teaching situation the student does not need to recognize a teacher's intention.  However, in the data that we have collected, there are many cases in which recognition is crucial to the advancement of a lesson. See utterance (13) in Figure \ref{Figure-scenario}}.  The goal will be achieved or, equivalently, the shared plan for the goal will be complete the teacher and student's beliefs about a lesson line up.   In Section \ref{sec:discourse-analysis} we discuss SharedPlans in more detail.
%interaction, we must understand what these constructs are, and how they emerge from the teacher's perspective.

% 11/28 - In a tutorial dialogue, a teacher's intentions must be understood by the student. Through these communicative actions, participants share beliefs and update their beliefs. teacher must update student's beliefs, and students must

